Decentralizing Information Technology: The Advent of Resource Based Systems

The growth of the Bitcoin network during the first decade of its operation to a global scale system is a singular event in the deployment of Information Technology systems. Can this approach serve as a wider paradigm for Information Technology services beyond the use case of digital currencies? We investigate this question by introducing the concept of resource based systems and their four fundamental characteristics: (i) resource-based operation, (ii) tokenomics, (iii) decentralized service provision, and (iv) rewards sharing. We explore these characteristics, identify design goals and challenges and investigate some crucial game theoretic aspects of reward sharing that can be decisive for their effective operation.

==> versions.tex <==
\newpage
{\small 
\begin{verbatim}
----------------------------
Version - Catalogue of changes
0.5  - first limited public release - Presentation at CBER Webinar. December 2nd 2021.
0.6  - various improvements to tokenomics section. first public release.
0.7  - inclusion of high-level blueprint section
0.75 - minor edits and improvements.
0.77 - typos and minor edits. 
\end{verbatim}
}

